Evaluating Fairness of Machine Learning Models Under Uncertain and Incomplete Information

Training and evaluation of fair classifiers is a challenging problem. This is partly due to the fact that most fairness metrics of interest depend on both the sensitive attribute information and label information of the data points. In many scenarios it is not possible to collect large datasets with such information. An alternate approach that is commonly used is to separately train an attribute classifier on data with sensitive attribute information, and then use it later in the ML pipeline to evaluate the bias of a given classifier. While such decoupling helps alleviate the problem of demographic scarcity, it raises several natural questions such as: how should the attribute classifier be trained?, and how should one use a given attribute classifier for accurate bias estimation? In this work we study this question from both theoretical and empirical perspectives. We first experimentally demonstrate that the test accuracy of the attribute classifier is not always correlated with its effectiveness in bias estimation for a downstream model. In order to further investigate this phenomenon, we analyze an idealized theoretical model and characterize the structure of the optimal classifier. Our analysis has surprising and counter-intuitive implications where in certain regimes one might want to distribute the error of the attribute classifier as unevenly as possible among the different subgroups. Based on our analysis we develop heuristics for both training and using attribute classifiers for bias estimation in the data scarce regime. We empirically demonstrate the effectiveness of our approach on real and simulated data.

==> Fairness under Uncertainty (ICML) (5)/experiment_arxiv.tex <==
\section{Perspective of the User of an Attribute Classifier}
\label{sec:experiments}


% In this section we explore the implications of the above theoretical analysis for the purposes of bias estimation when Assumption~I as defined in Eq.~\eqref{eq:cond_ind_assumption} holds or is expected to hold approximately. In particular, we explore a natural strategy, suggested by the above analysis, that the user of the attribute classifier can incorporate for better bias estimation if she has . 
% % We further study the sensitivity of these approaches to the conditional independence assumption. 

If the user of the attribute classifier expects Assumption~I as defined in Eq.~\eqref{eq:cond_ind_assumption} to (approximately) hold and she has some 
common data over $(y, a)$ 
from which she will  estimate the conditional errors~$g_1,g_2$ and the ratio of base rates~$r/s$, 
%due to 
exploiting 
\eqref{eq:bias_correction_formula}, she can try to improve the naive bias estimate $|\hat{\alpha}-\hat{\beta}|$ by dividing it by an estimate of the distortion factor~$\gamma$. In this section, we present an experiment that illustrates that such an approach indeed yields a better estimate of the true bias~$|\alpha-\beta|$. 
%and that 
In a data scarce regime, 
%it 
this approach 
also compares favorably to using the available data for directly estimating $|\alpha-\beta|$. 


\vspace{1mm}
\textbf{Dataset.~~}
% We study two real-world datasets  namely, , 
% as well as the Drug Consumption dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Drug+consumption+\%28quantified\%29}}. 
We use the FIFA~20 player dataset\footnote{\url{https://www.kaggle.com/stefanoleone992/fifa-20-complete-player-dataset}}.
We
%want to 
predict whether a soccer player's wage is above ($y=+1$) or below ($y=-1$) the median wage based on the player's age and their \emph{Overall} attribute. For doing so we train a one-hidden-layer NN. We restrict the dataset to contain only players of English or German nationality (leaving us with 2883 players) and consider nationality as sensitive attribute. We train an LSTM \cite{lstm} to predict this attribute from a player's name. 
% As 
% %also 
% suggested 
% %by 
% in 
% \cite{awasthi2019equalized}, 
In this case we can expect the conditional independence assumption~\eqref{eq:cond_ind_assumption} to hold since given a player's wage and nationality, their name should be conditionally independent of age and \emph{Overall} attribute.
Indeed, the measure proposed in \cite{awasthi2019equalized} 
%to evaluate 
%% to which extent the independence assumption~\eqref{eq:cond_ind_assumption} holds
%whether the independence assumption holds 
is small enough (see below) as to confirm that our expectation holds and the independence assumption is satisfied.




% \begin{itemize}
% \item Adult Dataset: 
%     % \item Drug Consumption Dataset (COMMENT MATT: SHOULD WE REMOVE EVERYTHING RELATED TO THE DRUG DATA SET?): We create a binary classification problem where the goal is to use the attributes of a user to predict if the person ever used the drug {\em Nicotine}.
%     % For this purpose we train a one layer neural network classifier using the following features: \textit{Age, Education, Country, Ethnicity, Escore, Oscore, Cscore, Impulsive, SS}. Again we fix this classifier to be used as our label classifier when estimating the bias.
%     % We train multiple attribute classifiers to predict the gender (``Male'' or ``Female'' as categorized in the dataset) using the following two features: \textit{Ascore, Nscore}.
%     \item FIFA~20 Player Dataset: 
    
% \vspace{-0.1in}
% \end{itemize}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=2.4in]{fig/est_bias_random_perturb.pdf}
%     \vspace{-0.1in}
%     \caption{Absolute difference between the estimated bias and the true bias, averaged over $10$ runs. COMMENT MATT: CHANGE LEGEND / LABEL OF y-AXIS AS SUGGESTED BY REVIEWER~#5}
%     \label{fig:est_bias_random_perturb}
% \end{figure}

%\subsection{Estimate Bias Under the Conditional Independence Assumption}
% The first setting we consider for bias estimation using label and attribute classifiers, is when the independence assumption~\eqref{eq:cond_ind_assumption} holds. This is the easiest setting in terms of how much common data is needed and how careful one needs to be in training the attribute classifier. In this scenario, Equation \eqref{eq:bias_correction_formula} holds and hence given an arbitrary attribute classifier, we can correct the estimate bias $|\hat{\alpha} - \hat{\beta}|$ by estimating the distortion factor $\gamma$~(as defined in \eqref{eq:def_E}) and using Equation \eqref{eq:bias_correction_formula}. Notice that in this scenario common data on $(a,y)$ is only needed to estimate $r = \mathbb{P}(y=1,a=1)$ and $s = \mathbb{P}(y=1, a=0)$ and $g_1, g_2$. These quantities can be estimated easily using a small amount of data. Furthermore, estimating $g_1, g_2$ only requires access to the attribute classifier (COMMENT MATT: WE ALSO NEED TO KNOW $y$??) and hence can be evaluated independently either by the designer of the attribute classifier, or by the user of the attribute classifier. Next, we empirically demonstrate that under the independence assumption, bias correction via \eqref{eq:bias_correction_formula} is an effective strategy. As mentioned before, on the UCI Adult dataset the label classifier is a Random Forest classifier ($100$ estimators with max depth $10$), which remains fixed during the whole experiment. In order to satisfy the independence assumption in \eqref{eq:cond_ind_assumption} we create attribute classifiers as follows. For a given $p \in (0.5,1)$ we create a random classifier $h$ where~(conditioned on the true attribute $a$) $h(x)=a$ with probability $p$, and $h(x)=1-a$ with probability $1-p$. It is an easy calculation to show that for such classifiers \eqref{eq:cond_ind_assumption} holds. Figure~\ref{fig:est_bias_random_perturb} shows the absolute difference between the estimated bias and the true bias, and we use two ways of estimating the bias: (a) Direct estimation using $|\hat{\alpha}-\hat{\beta}|$, and
% (b) Corrected bias estimation $|\hat{\alpha}-\hat{\beta}|/\gamma$, by using Equation~\eqref{eq:bias_correction_formula}.
% We can see that by correcting bias using $\gamma$, we get a much more accurate estimation of the true bias~$|\alpha-\beta|$. (COMMENT MATT: EXPLAIN HOW WE OBTAIN $\gamma$)


% \begin{figure}
%     \centering
%     \begin{overpic}[scale=0.38]{Fifa20Experiment_DiffEstSizes_NrRuns=100_NrTrain=1500_NrTest=1133_NrEstQ=[100 150 200 250].pdf}
%     \put(13.8,-4.5){\small {direct}}
%     %\put(33.6,-4.5){\small {corr.}}
%     \put(33.6,-4.5){\small $100$}
%     \put(52,-4.5){\small $150$}
%     \put(68,-4.5){\small $200$}
%     \put(86,-4.5){\small $250$}
%     \end{overpic}
    
%     \vspace{1mm}
%     \caption{Caption}
%     \label{fig:exp_fifa_dataset}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=5in]{fig/boxplot_adult.pdf}
    % \vspace{-0.05in}
     \caption{Experiment on the UCI Adult 
     dataset---independence 
     assumption~\eqref{eq:cond_ind_assumption} is violated.  Absolute difference between the true bias and the estimated bias for direct (Dir) and 
     %for 
     corrected~(Cor) estimation, when 
     100 to 1000 
     %bet. 100 and 1000 
     points of common data over $(y,a)$ are available, 
     and for naive (Naive)~estimation.}
     \label{fig:adult_bias_est}
%\vspace{-0.1in}
    % \caption{Absolute difference between the estimated bias and the true bias on the UCI Adult dataset. Boxplots are obtained from running the experiment for 100 times. The numbers represent different sample sizes used to estimate $r, s, g_1, g_2$. Naive: naive estimate ($|\hat{\alpha}-\hat{\beta}|$), Cor: Corrected estimate, Dir: Direct estimate over the common data of the given sample sizes.}\label{fig:adult_bias_est}
\end{figure*}

\vspace{1mm}
\textbf{Experimental setup.~~} We randomly split the dataset into three batches of sizes 1500, 1133 and 250, respectively. We use the first batch to train the label and the attribute classifier. On the second batch, we compute both the true bias~$|\alpha-\beta|$ and the \emph{naive estimate}~$|\hat{\alpha}-\hat{\beta}|$. Finally, we use $n\in\{100,150,200,250\}$ points from the third batch to estimate $g_1,g_2,r,s$, and thus $\gamma$, and also to directly estimate $|\alpha-\beta|$. We refer to the latter estimate as \emph{direct estimate}. Exploiting~\eqref{eq:bias_correction_formula}, we use the estimate of $\gamma$ to correct the naive estimate~$|\hat{\alpha}-\hat{\beta}|$ by dividing it by the estimate of $\gamma$. We refer to the 
result 
%resulting estimate 
as \emph{corrected estimate}. 

Figure~\ref{fig:exp_fifa_dataset} shows the absolute difference between the true bias and the various estimates, where for the direct estimate and the corrected estimate we show the results depending on $n$, the amount of data for which we have both $y$ and $a$. The boxplots are obtained from running the experiment  100 times. 
We can see that the corrected estimate significantly improves over the naive estimate (e.g., the mean absolute difference, averaged over the 100 runs, is 0.0831 for the naive estimate and 0.0461 for the corrected estimate 
%when using $n=250$ points).
with 
%when 
$n=250$). 
Furthermore, the corrected estimate consistently outperforms the direct estimate. When %there are 
only $n=100$ points of common data over $(y,a)$ 
%available, 
are used, 
the mean absolute difference for the corrected estimate is 0.054 while for the direct estimate it is 0.0837. 
%This shows that ...
%
In this experiment, the mean true bias 
%$|\alpha-\beta|$ 
is 0.14, the mean error of the label and the attribute classifier is 0.18 and 0.25, respectively, and the mean violation of the independence assumption according to the measure proposed in \cite{awasthi2019equalized} is $0.017$.



\subsection{An Active Sampling based Algorithm for Bias Estimation in General Settings}
\label{sec:active_sampling}
In some real-world scenarios the conditional independence assumption might be violated, and we would like to ask, in those cases, does the correction as specified in Eq.~\eqref{eq:bias_correction_formula} still give a good estimate of the true bias? 
We show in the following that the correction might not always lead to a better bias estimate when Assumption I does not hold.
Therefore, in order to obtain a good bias estimate in general, we explore active-sampling strategies that aim to use as little common data over $(y,a)$ as possible, ideally comparable to the setting when the independence assumption holds.

\vspace{1mm}
\textbf{Dataset.~~} We use the UCI Adult dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Adult}}, which comes divided into a training and a test set.
On the training set, we train Random Forest classifiers for both predicting the label (income: $>50K$ or not, using all features present in the dataset except gender) and the attribute (gender: ``Male'' or ``Female'' as categorized in the dataset, using all features except income). 
% We fix this classifier to be used as our label classifier and study the problem of estimating the bias, as defined in \eqref{eq:equal-opportunity}, of the classifier.
%We did a statistical conditional independence test over this dataset and found that the conditional independence assumption fails to hold. 
We used the measure proposed in \cite{awasthi2019equalized} to evaluate 
% to which extent the independence assumption~\eqref{eq:cond_ind_assumption} holds
whether the independence assumption~\eqref{eq:cond_ind_assumption} (approximately) holds and found that 
%it 
the independence assumption clearly fails to hold. 

\paragraph{Inaccurate bias estimation when the conditional independence assumption is violated.}
We use the UCI Adult training set for training our label classifier and attribute classifier. For the Adult test set (around 16,000 examples), we hold out a set with $2,000$ examples for estimating $g_1, g_2, r, s$ since it requires some common data over $(y, a)$, and use the rest for estimating the true bias ($|\alpha-\beta|$).
In Figure~\ref{fig:adult_bias_est}, we show the absolute difference between the estimated bias and the true bias.
For the estimated bias, we use the same setting as the previous experiment, with direct estimate, corrected estimate, and naive estimate.
We can see the the correction gives a more accurate estimate than direct estimation, however, the naive estimate remains to be the one with the most accurate estimate.



% \begin{figure*}[h]
% \centering
% \subcaptionbox{By \textit{post-processing} the attribute classifier.
% \label{fig:sensitivity_post}}
% {\includegraphics[width=2in]{fig/post_processing_adult.pdf}
% % \hspace{-0.1in}
% % \includegraphics[width=1.7in]{fig/post_processing_drug.pdf}
% }
% \hspace{0.2in}
% \subcaptionbox{By \textit{class re-weighting} when training the attribute classifier.
% \label{fig:sensitivity_reweight}}
% {\includegraphics[width=2in]{fig/reweight_adult.pdf}
% % \hspace{-0.1in}
% % \includegraphics[width=1.7in]{fig/reweight_drug.pdf}
% }
% \caption{Sensitivity analysis over the estimated bias $\hat{\alpha}-\hat{\beta}$, corrected bias $(\hat{\alpha}-\hat{\beta})/\gamma$, and the true bias $\alpha-\beta$, by different intervention strategies on the Adult dataset.}
% % \vspace{-0.1in}
% \end{figure*}

% \noindent \textbf{Intervention for the Label Classifier.} From the label classifier's perspective, without making any assumptions on the attribute classifier, a natural approach is to still use \eqref{eq:bias_correction_formula} to correct the estimated bias. One could then quantify the error in the corrected bias estimates to the degree to which the independence assumption is violated. The advantage of this approach is that the common data requirement is the same as the one in the case when the independence assumption holds. We implement this approach where the label classifier uses the given attribute classifier $h$ and picks a threshold $\theta_a$ using which the dataset is labeled with attribute information. In particular, we have that
% % Common approaches for improving the fairness metrics include calibrating/post-processing the classifier with varying thresholds, or re-weight classes in the training process to balance different classes.
% % In this section, we present experiments on both UCI Adult dataset and the Drug consumption dataset, and show that when the conditional independence assumption is violated, the corrected bias estimation is very sensitive to various post-processing thresholds and class-reweighting algorithms.
% % \paragraph{Post-processing}   
% % One way to balance different classes is by post-processing predictions from the attribute classifier by varying thresholds. Formally, given an attribute classifier $h$ with a probability estimation $P(h(x)=a)$, we can post-process the data by varying the threshold $\theta_a$, i.e., 
% $\hat{h}(x) = a, \text{ if } \mathbb{P}(h(x)=a) > \theta_a$.
% One can then estimate the bias using the predicted attributes and correct them using \eqref{eq:bias_correction_formula}. In Figure~\ref{fig:sensitivity_post} (left), we show how the estimated bias, corrected bias change with respect to different post-processing thresholds, over the output of a Random Forest attribute classifier, on the UCI Adult dataset. As can be seen the corrected bias is very sensitive to the threshold $\theta_a$, when the conditional independence assumption fails to hold.


% We next show that even when the independence assumption approximately holds, the approach does not lead to better bias estimation. For this purpose we use the Drug Consumption dataset where the independence assumption is known to hold approximately \cite{awasthi2019equalized}. As can be seen from Figure~\ref{fig:sensitivity_post} (right), even in this case the correct bias in general does not lead to better estimates and is sensitive to the threshold used. This suggests that from the label classifier's point of view, one needs to use more common data about $(y,a)$ in order to accurately estimate bias. We next explore whether interventions on the attribute classifier can alleviate this.
% % shows the sensitivity of the estimated bias, corrected bias compared to the true bias over the drug consumption dataset, by a Logistic Regression classifier over the attribute and post-processing the classifier output using different thresholds.

% \noindent \textbf{Intervention for the Attribute Classifier.}
% From the perspective of the attribute classifier, Theorem~\ref{thm:opt-classifier} suggests that one should consider reweighing of the examples belonging to different sensitive attributes, in an unequal manner. We investigate the effectiveness of this strategy for training the attribute classifier and then using the trained classifier for bias correction via \eqref{eq:bias_correction_formula}.
% % Another common way to balance difference classes during the training process is by re-weighting the loss over different attribute classes.
% Figures~\ref{fig:sensitivity_reweight} shows the sensitivity of the corrected bias with respect to different class weights used when training the attribute classifier, for the Adult dataset and the Drug Consumption dataset, respectively. To train the attribute classifier, we use a Logistic Regression model with varying weights over each class of the sensitive attribute (indicated by the x-axis in the figures).

% As can be seen again, the estimated bias does not always accurately approximate the true bias, even on the Drug Consumption dataset where the conditional independence assumption holds approximately. This suggests that in general, even when the independence assumption is slightly violated, one needs to use more data to accurately estimate the bias. This raises the natural question of designing sampling heuristics that can estimate the bias using little overhead, as compared to the case when the independence assumption holds. In the next section we propose a general heuristic for this purpose. 
\paragraph{Active sampling algorithm.}
\label{sec:active}
We next address the limitations of the approaches explored above.
% that are sensitive to the conditional independence assumption. 
In particular, we propose a \emph{general active-sampling} based strategy that the label classifier can use to accurately estimate the bias, using as little common data over $(y,a)$ as possible, given the attribute classifier. Furthermore, we will make \emph{no assumption} about the conditional independence or the structure of the attribute classifier.
% As we see from the previous section, the corrected bias estimation is sensitive when the conditional independence assumption fails to hold.
% Hence in this section we propose an active learning approach to better estimate the bias without the conditional independence assumption.
% Our setting is as follows: assume we're given an attribute classifier, and would like to build the label classifier. We could actively query some true attributes $a$ for some samples, and the goal is to best estimate the bias $|\alpha-\beta|$. 

In the general setting the estimated bias and the true bias are related as 
%the following:
follows:
\begin{theorem}
\label{thm:opt-classifier-general}
The true bias $\alpha-\beta$ can be derived from $\hat{\alpha}, \hat{\beta}$ as:
\begin{align}
\alpha-\beta 
&=\frac{\hat{\alpha}(\frac{s}{r}g_1+1-g_2)(1-\delta_1+\frac{r}{s}\delta_2)}{1-\delta_1-\delta_2} \nonumber \\ 
&- 
\frac{\hat{\beta}(1-g_1+\frac{r}{s}g_2)(1+\frac{s}{r}\delta_1-\delta_2)}{1-\delta_1-\delta_2},
\label{eq:true-bias-updates}
\end{align}
where 
\begin{align}
\label{eq:delta-def}
    \delta_1 &= \mathbb{P}(\hat{a}=1 | f(x)=1, a=0, y=1), \nonumber \\
    \delta_2 &= \mathbb{P}(\hat{a}=0 | f(x)=1, a=1, y=1),
\end{align}
and $g_1, g_2$ are as defined in Eq.~\eqref{eq:cond-error-def}. 
\end{theorem}



\begin{figure*}[t]
\centering
\includegraphics[width=2.7in]{fig/al_est.pdf}
\hspace{1.2cm}
\includegraphics[width=2.65in]{fig/al_direct_est.pdf}
    % \vspace{-0.15in}
    \caption{The absolute difference between estimated bias and the true bias, based on different \textbf{active sampling} strategies (left), and based on \textbf{direct estimation} over selected samples using uniform/positive sampling (right). Both are results averaged over $10$ runs with random initialization.}
    \label{fig:active_learning_bias_est}
% \vspace{-0.1in}
\end{figure*}




% \begin{proof}
% To see \eqref{eq:true-bias-updates} notice that from the definition of $\hat{\alpha}$, we have
% \begin{align}
% \label{eq:intermediate}
%     \hat{\alpha} &= \mathbb{P}(f(x)=1 | y=1, \hat{a}=1) = \frac{\mathbb{P}(f(x)=1, y=1, \hat{a}=1)}{\mathbb{P}(y=1, \hat{a}=1)}\nonumber\\ 
%     &= \frac{\mathbb{P}(a=0, f(x)=1, y=1, \hat{a}=1) + \mathbb{P}(a=1, f(x)=1, y=1, \hat{a}=1)}
%     {\mathbb{P}(y=1, a=0, \hat{a}=1) + \mathbb{P}(y=1, a=1, \hat{a}=1)}
%     \end{align}
% %     &= \frac{P(\hat{a}=1|f(x)=1, a=0, y=1)P(f(x)=1|a=0,y=1)P(a=0,y=1)}
% %     {P(\hat{a}=1| y=1, a=0)P(y=1, a=0) + P(\hat{a}=1| y=1, a=1)P(y=1, a=1)}\\
% %     &\quad+ \frac{P(\hat{a}=1|f(x)=1, a=0, y=1)P(f(x)=1|a=0,y=1)P(a=0,y=1)}
% %     {P(\hat{a}=1| y=1, a=0)P(y=1, a=0) + P(\hat{a}=1| y=1, a=1)P(y=1, a=1)}\\
% %     &= \frac{\delta_1 \beta s + (1-\delta_2)\alpha r}{g_1 s + (1-g_2) r},
% % \end{align*}
% Next we first simplify the two terms in the numerator. We can write
% \begin{align*}
%     &\mathbb{P}(a=0, f(x)=1, y=1, \hat{a}=1) \\
%     &= \mathbb{P}(\hat{a}=1|f(x)=1, a=0, y=1)\mathbb{P}(f(x)=1|a=0,y=1)\mathbb{P}(a=0,y=1)\\
%     &= \delta_1 \beta s.
% \end{align*}
% Similarly, we write
% \begin{align*}
%     &\mathbb{P}(a=1, f(x)=1, y=1, \hat{a}=1) \\
%     &= \mathbb{P}(\hat{a}=1|f(x)=1, a=1, y=1) \mathbb{P}(f(x)=1|a=1,y=1)\mathbb{P}(a=1,y=1)\\
%     &= (1-\delta_2) \alpha r.
% \end{align*}
% For the denominator we have
% \begin{align*}
%     \mathbb{P}(y=1, a=0, \hat{a}=1) &= \mathbb{P}(\hat{a}=1| y=1, a=0)P(y=1, a=0)\\
%     &= g_1 s.
% \end{align*}
% Similarly, we have
% \begin{align*}
%     \mathbb{P}(y=1, a=1, \hat{a}=1) &= \mathbb{P}(\hat{a}=1| y=1, a=1)P(y=1, a=1)\\
%     &= (1-g_2) r.
% \end{align*}
% Substituting into \eqref{eq:intermediate} we get
% \begin{align*}
%     \hat{\alpha} &= \frac{\delta_1 \beta s + (1-\delta_2)\alpha r}{g_1 s + (1-g_2) r}.
% \end{align*}
% Similarly for $\hat{\beta}$, it is easy to derive:
% \begin{align*}
%     \hat{\beta} &= \mathbb{P}(f=1 | y=1, \hat{a}=0) = \frac{\delta_2 \alpha r + (1-\delta_1)\beta s}{(1-g_1) s + g_2 r}.
% \end{align*}
% Hence we have:
% \begin{align}
%     \hat{\alpha}[g_1 \frac{s}{r}  + (1-g_2)] = \delta_1  \frac{s}{r} \beta + (1-\delta_2) \alpha,
% \label{eq_alpha}
% \end{align}
% \vspace{-0.1in}
% \begin{align}
%     \hat{\beta}[(1-g_1) + g_2 \frac{r}{s}] = \delta_2 \frac{r}{s} \alpha + (1-\delta_1)\beta.
% \label{eq_beta}
% \end{align}

% Multiplying Eq.~\eqref{eq_alpha} by $(1-\delta_1+\frac{r}{s}\delta_2)$, multiplying Eq.~\eqref{eq_beta} by $(1+\frac{s}{r}\delta_1-\delta_2)$, and subtracting the latter from the former, we get:
% \begin{align*}
% &(1-\delta_1-\delta_2)(\alpha-\beta) =\\
% &\hat{\alpha}[g_1 \frac{s}{r}  + (1-g_2)](1-\delta_1+\frac{r}{s}\delta_2) - \hat{\beta}[(1-g_1) + g_2 \frac{r}{s}](1+\frac{s}{r}\delta_1-\delta_2).
% \end{align*}
% Dividing the right hand side by $1-\delta_1-\delta_2$ we have Eq.~\eqref{eq:true-bias-updates}.
% \end{proof}


\begin{algorithm}
\caption{Active Sampling}
\begin{algorithmic}[1]
\item[] \textbf{Input:} $D_2 = \{(x_1, y_1), \dots, (x_m, y_m)\}$, attribute classifier $h$, parameters $b, w$.
\item [] \textbf{Output:} Estimated bias $|\hat{\alpha} - \hat{\beta}|$, tolerance $\epsilon$.
\STATE Sample a set of $b$ examples uniformly at random from $D_2$ conditioned on $y=1$ and get their true attributes. Get estimates $\hat{r}$ and $\hat{s}$ using the sampled examples.
\STATE Initialize $t=0$ and $g^{(0)}_1, g^{(0)}_2, \delta^{(0)}_1, \delta^{(0)}_2$ to be zero.
\FOR{$t=1, \dots$}
\STATE Sample a batch of $b$ unlabeled~(i.e. no sensitive attribute information) examples uniformly at random from $D_2$ conditioned on $y=1$.
\STATE Sort the examples in ascending order according to the uncertainty of $h$, i.e., $|h(x)-0.5|$.
\STATE Obtain true attribute information the first $w$ examples and append to the labeled set of data. Compute $g^{(t+1)}_1, g^{(t+1)}_2, \delta^{(t+1)}_1, \delta^{(t+1)}_2$ on the labeled set using \eqref{eq:cond-error-def} and \eqref{eq:delta-def}. 
\STATE If $|g_1^{(t+1)} - g_1^{(t)}|, |g_2^{(t+1)} - g_2^{(t)}|, |\delta_1^{(t+1)} - \delta_1^{(t)}|, |g\delta_2^{(t+1)} - \delta_2^{(t)}|$ are all bounded by $\epsilon$ then \textbf{break}.
\ENDFOR
\STATE Output estimated bias obtained by using \eqref{eq:true-bias-updates} and the above estimates.
\end{algorithmic}
\label{alg:active-sampling}
\end{algorithm}


While $r,s$ can be estimated from a small amount of data, we explore sampling strategies for estimating the attribute classifier dependent quantities, namely, $g_1, g_2$ and $\delta_1, \delta_2$. Two natural sampling schemes are: 
% We initialize with a uniformly sampled $100$ examples, and then start querying more samples in a batch of $100$ examples in each iteration. We experiment with 
(i) {\em Uniform sampling} where we uniformly sample a set of examples and get their true sensitive attribute information, and (ii) {\em Positive sampling}: where we perform uniform sampling on the subset of examples with $y=1$. We expect positive sampling to perform better than uniform sampling, since the quantities that we are estimating are conditioned on $y=1$. We compare the above two approaches with (iii) an {\em active sampling} approach that involves querying for true sensitive attributes~(conditioned on $y=1$) of examples on which the attribute classifier is the most uncertain (as described in Algorithm~\ref{alg:active-sampling}).
% sampling from the subset where $y=1$; (3) \textbf{Uncertainty sampling}: sampling  from the subset where $y=1$ with $P(h(x)=a)$ closest to $0.5$. 
For each of the methods, in each iteration, we compute the estimated bias on the UCI Adult test set by using true values of $a$ over the selected samples, and the predicted values $\hat{a}$ from the attribute classifier for the unselected samples, using a sampling batch size of $100$. 
%
The results are shown in Figure~\ref{fig:active_learning_bias_est} (left), where we see that the uncertainty based active sampling approach requires significantly less common data to accurately estimate the~bias.
% Figures~\ref{fig:active_learning_g_and_delta} shows the performance of our sampling scheme on estimating $g_1, g_2$ and $\delta_1, \delta_2$ respectively. 



Furthermore, we also compare our approach with (iv) {\em Direct estimation}: where we directly estimate the bias~($|\alpha-\beta|$) based on the currently sampled set $S$, i.e., the small amount of common $(y, a)$ on the same test set, using a uniform sampling strategy and a positive sampling strategy. The result is shown in Figure~\ref{fig:active_learning_bias_est} (right). Note that the magnitude in the y-axis is much larger compared to the left figure, indicating that direct estimation using few samples tends to give less reliable estimation of the bias.



% The absolute difference between the estimated bias and the true bias is shown  in Figure~\ref{fig:active_learning_bias}, using active sampling strategy (1)-(3).

% In Figure~\ref{fig:active_learning_g} and Figure~\ref{fig:active_learning_delta}, we also show the estimate of $g_1, g_2$, as well as $\delta_1, \delta_2$, under different active sampling strategies.



% \begin{figure}[h]
% \centering
%     \includegraphics[width=1.3in]{fig/al_g1.pdf}
%     \includegraphics[width=1.3in]{fig/al_g2.pdf}
%     \includegraphics[width=1.3in]{fig/al_d1.pdf}
%     \includegraphics[width=1.3in]{fig/al_d2.pdf}
%     \caption{Estimation of $g_1, g_2$ (left two figures) and $\delta_1, \delta_2$ (right two figures) under different active sampling strategies. The solid black line is the true value of $g_1, g_2$ and $\delta_1, \delta_2$.}
%     \label{fig:active_learning_g_and_delta}
% % \vspace{-0.1in}
% \end{figure}


